Code Needs Comments: Enhancing Code LLMs with Comment Augmentation

The programming skill is one crucial ability for Large Language Models (LLMs), necessitating a deep understanding of programming languages (PLs) and their correlation with natural languages (NLs). We examine the impact of pre-training data on code-focused LLMs' performance by assessing the comment density as a measure of PL-NL alignment. Given the scarcity of code-comment aligned data in pre-training corpora, we introduce a novel data augmentation method that generates comments for existing code, coupled with a data filtering strategy that filters out code data poorly correlated with natural language. We conducted experiments on three code-focused LLMs and observed consistent improvements in performance on two widely-used programming skill benchmarks. Notably, the model trained on the augmented data outperformed both the model used for generating comments and the model further trained on the data without augmentation.

==> Tables/llama_result.tex <==
\begin{table*}[ht]
\centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{llllllll}
\hline % pass@1 采用的 greedy 结果
\multirow{2}{*}{Model} & \multirow{2}{*}{DATA}                               & \multicolumn{3}{c}{humaneval}              & \multicolumn{3}{c}{MBPP}          \\
                       &                                                     & pass@1 & pass@5 & pass@10               & pass@1 & pass@5    & pass@10  \\ \hline
Llama2                  & \multicolumn{1}{l|}{SPCA} & 16.46   & 27.87   & \multicolumn{1}{l|}{34.22} & 19   & 40.1   & 48.16       \\ % 8000
Llama2                  & \multicolumn{1}{l|}{SPO}        & 17.07   & 31.09     & \multicolumn{1}{l|}{39.06} & 20.4   & 52.45   & 50.9       \\ % 9000
Llama2                  & \multicolumn{1}{l|}{SPCS}    & (19.51)   & -   & \multicolumn{1}{l|}{-} & (30.6)   & -   & -       \\ % 还在跑

\hline
\end{tabular}
    }
    \caption{llama result}
    \label{llama_result}
\end{table*}
